Gathering dust: A galaxy-wide study of dust emission from cloud complexes in NGC 300

We used multi-band observations by the Herschel Space Observatory to study the dust emission properties of the nearby spiral galaxy NGC 300. We compiled a first catalogue of the population of giant dust clouds (GDCs) in NGC 300 and give an estimate of the total dust mass of the galaxy. We carried out source detection with the multiwavelength source extraction algorithm getsources and calculated physical properties of the GDCs, including mass and temperature, from five-band Herschel PACS and SPIRE observations from 100-500 $\mu$m; the final size and mass estimates are based on the observations at 250 $\mu$m that have an effective spatial resolution of $\sim$170 pc. We correlated our final catalogue of GDCs to pre-existing catalogues of HII regions to infer the number of GDCs associated with high-mass star formation and determined the H$\alpha$ emission of the GDCs. Our final catalogue of GDCs includes 146 sources, 90 of which are associated with known HII regions. We find that the dust masses of the GDCs are completely dominated by the cold dust component and range from $\sim$1.1$\cdot$10$^{3}$ - 1.4$\cdot$10$^{4}$ M$_{\odot}$. The GDCs have effective temperatures of $\sim$13-23 K and show a distinct cold dust effective temperature gradient from the centre towards the outer parts of the stellar disk. We find that the population of GDCs in our catalogue constitutes $\sim$16% of the total dust mass of NGC 300, which we estimate to be about 5.4$\cdot$10$^{6}$ M$_{\odot}$. At least about 87% of our GDCs have a high enough average dust mass surface density to provide sufficient shielding to harbour molecular clouds. We compare our results to previous pointed molecular gas observations in NGC 300 and results from other nearby galaxies and also conclude that it is very likely that most of our GDCs are associated with complexes of giant molecular clouds.

==> symbols.tex <==
% Local symbols
\newcommand{\kb}{k_{\mathrm{B}}}
\newcommand{\msun}{M$_\text{\odot}$}
\newcommand{\rsun}{R_{\odot}}
\newcommand{\lsun}{L_{\odot}}
\newcommand{\avir}{\alpha_{\mathrm{vir}}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\veck}{\mathbf{k}}
\newcommand{\vecB}{\mathbf{B}}
\newcommand{\vecf}{\mathbf{f}}
\newcommand{\nhat}{\hat{\mathbf{n}}}
\newcommand{\vecS}{\mathbf{S}}
\newcommand{\vecI}{\mathbf{I}}
\newcommand{\vecPi}{\boldsymbol{\Pi}}
\newcommand{\vecT}{\mathbf{T}}
\newcommand{\veco}{{\bm \Omega}}
\newcommand{\ehat}{\hat{\mathbf{e}}}
\newcommand{\alphab}{\alpha_{\mathrm{B}}}

% AAStex symbols
\usepackage{amssymb}

% Journals
\newcommand{\physrep}{Phys.~Rep.}
\newcommand{\aapr}{Astron.\& Astrophys.~Rev.}
\newcommand{\aap}{Astron.~\& Astrophys.}
\newcommand{\aaps}{Astron.~\& Astrophys.~Supp.}
\newcommand{\apj}{Astrophys.~J.}
\newcommand{\apjs}{Astrophys.~J.~Supp.}
\newcommand{\apjl}{Astrophys.~J.}
\newcommand{\apss}{Astrophys.~\& Space~Science}
\newcommand{\aj}{Astron.~J.}
\newcommand{\araa}{Annu.~Rev.~Astron.~Astrophys.}
\newcommand{\pasp}{Proc.~Astron.~Soc.~Pac.}
\newcommand{\mnras}{Mon.~Not.~Roy.~Astron.~Soc.}
\newcommand{\pasj}{Proc.~Astron.~Soc.~Japan}
\newcommand{\nat}{Nature}
